Dissipative Channels Determine Open Electromagnetic Quantization

We formulate a quantization scheme for open electromagnetic systems with arbitrary passive boundary conditions. Rather than specifying reservoirs phenomenologically, the method identifies them from the dissipation geometry of the Maxwell operator. Factoring the imaginary part of the Maxwell operator gives a bosonic realization of the field operator and separates the fluctuation channels into medium-assisted reservoirs from material absorption and boundary-assisted reservoirs from exchange through the open boundary. Depending on the boundary condition, the latter become free-space radiation modes, impedance-load channels, guided port modes, or more general boundary channels. Green-function input-output relations then follow as an application, yielding frequency-dependent scattering and noise kernels without Markov or single-mode assumptions. To illustrate the practical application, we consider a lossy structure with mixed impedance and outgoing boundaries, and photonic integrated circuit configurations with waveguide port boundaries.

==> sorsamp2.tex <==
@article{PRA_twophotoncoherence_2016,
  title = {Quantum coherence of light emitted by two single-photon sources in a structured environment},
  author = {Canaguier-Durand, Antoine and Carminati, R\'emi},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {3},
  pages = {033836},
  numpages = {5},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.033836},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.033836}
}
@article{Shen_PRL_twophoton_2007,
  title = {Strongly Correlated Two-Photon Transport in a One-Dimensional Waveguide Coupled to a Two-Level System},
  author = {Shen, Jung-Tsung and Fan, Shanhui},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {15},
  pages = {153003},
  numpages = {4},
  year = {2007},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.153003},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.153003}
}
@article{Roy_PRL_twophoton_2011,
  title = {Two-Photon Scattering by a Driven Three-Level Emitter in a One-Dimensional Waveguide and Electromagnetically Induced Transparency},
  author = {Roy, Dibyendu},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {5},
  pages = {053601},
  numpages = {4},
  year = {2011},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.053601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.053601}
}

@article{Fan_PRA_fewphoton_2015,
  title = {Input-output formalism for few-photon transport: A systematic treatment beyond two photons},
  author = {Xu, Shanshan and Fan, Shanhui},
  journal = {Phys. Rev. A},
  volume = {91},
  issue = {4},
  pages = {043845},
  numpages = {11},
  year = {2015},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.91.043845},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.91.043845}
}

@article{Lodahl_RevModPhy_nanostructure_2015,
  title = {Interfacing single photons and single quantum dots with photonic nanostructures},
  author = {Lodahl, Peter and Mahmoodian, Sahand and Stobbe, S\o{}ren},
  journal = {Rev. Mod. Phys.},
  volume = {87},
  issue = {2},
  pages = {347--400},
  numpages = {54},
  year = {2015},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.87.347},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.87.347}
}

@article{Dowran_Laserphotonics_nanocavity_2025,
author = {Dowran, Mohammadjavad and Kilic, Ufuk and Lamichhane, Suvechhya and Erickson, Adam and Barker, Joshua and Schubert, Mathias and Liou, Sy-Hwang and Argyropoulos, Christos and Laraoui, Abdelghani},
title = {Plasmonic Nanocavity to Boost Single Photon Emission From Defects in Thin Hexagonal Boron Nitride},
journal = {Laser \& Photonics Reviews},
volume = {19},
number = {3},
pages = {2400705},
keywords = {hexagonal boron nitride, metal nanocavity, plasmon, Purcell effect, single photon emitters},
doi = {https://doi.org/10.1002/lpor.202400705},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.202400705},
year = {2025}
}


@article{Ye_PRL_Coldatom_2023,
  title = {Universal Quantum Optimization with Cold Atoms in an Optical Cavity},
  author = {Ye, Meng and Tian, Ye and Lin, Jian and Luo, Yuchen and You, Jiaqi and Hu, Jiazhong and Zhang, Wenjun and Chen, Wenlan and Li, Xiaopeng},
  journal = {Phys. Rev. Lett.},
  volume = {131},
  issue = {10},
  pages = {103601},
  numpages = {6},
  year = {2023},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.131.103601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.131.103601}
}
@article{Tame2013,
  title = {Quantum plasmonics},
  volume = {9},
  ISSN = {1745-2481},
  url = {http://dx.doi.org/10.1038/nphys2615},
  DOI = {10.1038/nphys2615},
  number = {6},
  journal = {Nature Physics},
  publisher = {Springer Science and Business Media LLC},
  author = {Tame,  M. S. and McEnery,  K. R. and \"{O}zdemir,  Ş. K. and Lee,  J. and Maier,  S. A. and Kim,  M. S.},
  year = {2013},
  month = jun,
  pages = {329–340}
}

@article{Sheremet_RMP_waveguideQED_2023,
  title = {Waveguide quantum electrodynamics: Collective radiance and photon-photon correlations},
  author = {Sheremet, Alexandra S. and Petrov, Mihail I. and Iorsh, Ivan V. and Poshakinskiy, Alexander V. and Poddubny, Alexander N.},
  journal = {Rev. Mod. Phys.},
  volume = {95},
  issue = {1},
  pages = {015002},
  numpages = {59},
  year = {2023},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.95.015002},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.95.015002}
}
@article{Mahmoodian_PRL_waveguide_2018,
  title = {Strongly Correlated Photon Transport in Waveguide Quantum Electrodynamics with Weakly Coupled Emitters},
  author = {Mahmoodian, Sahand and \ifmmode \check{C}\else \v{C}\fi{}epulkovskis, Mantas and Das, Sumanta and Lodahl, Peter and Hammerer, Klemens and S\o{}rensen, Anders S.},
  journal = {Phys. Rev. Lett.},
  volume = {121},
  issue = {14},
  pages = {143601},
  numpages = {6},
  year = {2018},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.121.143601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.121.143601}
}
@article{Slussarenko_APL_Photonic_2019,
    author = {Slussarenko, Sergei and Pryde, Geoff J.},
    title = {Photonic quantum information processing: A concise review},
    journal = {Applied Physics Reviews},
    volume = {6},
    number = {4},
    pages = {041303},
    year = {2019},
    month = {10},
}



@article{Thomas2022,
  title = {Efficient generation of entangled multiphoton graph states from a single atom},
  volume = {608},
  ISSN = {1476-4687},
  url = {http://dx.doi.org/10.1038/s41586-022-04987-5},
  DOI = {10.1038/s41586-022-04987-5},
  number = {7924},
  journal = {Nature},
  publisher = {Springer Science and Business Media LLC},
  author = {Thomas,  Philip and Ruscio,  Leonardo and Morin,  Olivier and Rempe,  Gerhard},
  year = {2022},
  month = aug,
  pages = {677–681}
}

@article{de_RMP_nonMarkovian_2018,
  title = {Dynamics of non-Markovian open quantum systems},
  author = {de Vega, In\'es and Alonso, Daniel},
  journal = {Rev. Mod. Phys.},
  volume = {89},
  issue = {1},
  pages = {015001},
  numpages = {58},
  year = {2017},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.89.015001},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.89.015001}
}

@article{Gonz_PRA_nonMarkovian_2017,
  title = {Markovian and non-Markovian dynamics of quantum emitters coupled to two-dimensional structured reservoirs},
  author = {Gonz\'alez-Tudela, A. and Cirac, J. I.},
  journal = {Phys. Rev. A},
  volume = {96},
  issue = {4},
  pages = {043811},
  numpages = {20},
  year = {2017},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.96.043811},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.96.043811}
}
@article{psiquantum_2025,
  title = {A manufacturable platform for photonic quantum computing},
  volume = {641},
  ISSN = {1476-4687},
  url = {http://dx.doi.org/10.1038/s41586-025-08820-7},
  DOI = {10.1038/s41586-025-08820-7},
  number = {8064},
  journal = {Nature},
  publisher = {Springer Science and Business Media LLC},
  month = feb,
  pages = {876–883}
}

@article{Choi_PRApplied,
  title = {Non-Markovian analysis of atom-field interactions in dissipative electromagnetic environments},
  author = {Choi, Hyunwoo and Roth, Thomas E. and Chew, Weng C. and Na, Dong-Yeop},
  journal = {Phys. Rev. Appl.},
  volume = {24},
  issue = {4},
  pages = {044056},
  numpages = {21},
  year = {2025},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/kvxk-sp94},
  url = {https://link.aps.org/doi/10.1103/kvxk-sp94}
}
@misc{Choi_twoquanta,
      title={Computational framework for non-Markovian multi-emitter dynamics beyond the single-excitation limit}, 
      author={Hyunwoo Choi and Weng Cho Chew and Dong-Yeop Na},
      year={2026},
      eprint={2604.02741},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2604.02741}, 
}
@misc{Choi_FDTDQE,
      title={Atom-Field Non-Markovian Dynamics in Open and Dissipative Systems: An Efficient Memory-Kernel Approach Linked to Dyadic Greens Function and CEM Treatments}, 
      author={Hyunwoo Choi and Jisang Seo and Weng C. Chew and Dong-Yeop Na},
      year={2025},
      eprint={2511.03561},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2511.03561}, 
}
@article{Vidal_PRL_fewmode_2021,
  title = {Few-Mode Field Quantization of Arbitrary Electromagnetic Spectral Densities},
  author = {Medina, Ivan and Garc\'{\i}a-Vidal, Francisco J. and Fern\'andez-Dom\'{\i}nguez, Antonio I. and Feist, Johannes},
  journal = {Phys. Rev. Lett.},
  volume = {126},
  issue = {9},
  pages = {093601},
  numpages = {7},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.126.093601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.126.093601}
}
@book{gerry2023introductory,
  title={Introductory quantum optics},
  author={Gerry, Christopher C and Knight, Peter L},
  year={2023},
  publisher={Cambridge university press}
}

@article{Monica2022ECM,
url = {https://doi.org/10.1515/nanoph-2021-0795},
title = {Few-mode field quantization for multiple emitters},
title = {},
author = {Mónica Sánchez-Barquilla and Francisco J. García-Vidal and Antonio I. Fernández-Domínguez and Johannes Feist},
pages = {4363--4374},
volume = {11},
number = {19},
journal = {Nanophotonics},
doi = {doi:10.1515/nanoph-2021-0795},
year = {2022},
lastchecked = {2025-12-02}
}
@BOOK{Scully1997quantum,
  author        = {M. O. Scully and M. S. Zubairy},
  title         = {Quantum Optics},
  publisher     = {Cambridge University Press},
  year          = {1997}
}
@BOOK{Mandel1995optical,
  author        = {L. Mandel and E. Wolf},
  title         = {Optical Coherence and Quantum Optics},
  publisher     = {Cambridge University Press},
  year          = {1995}
}

@article{Na2021cqNMD,
  title = {Diagonalization of the Hamiltonian for finite-sized dispersive media: Canonical quantization with numerical mode decomposition},
  author = {Na, Dong-Yeop and Zhu, Jie and Chew, Weng C.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {6},
  pages = {063707},
  numpages = {15},
  year = {2021},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.063707},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.063707}
}

@article{Na2023quantumEMLossy,
  title = {Numerical framework for modeling quantum electromagnetic systems involving finite-sized lossy dielectric objects in free space},
  author = {Na, Dong-Yeop and Roth, Thomas E. and Zhu, Jie and Chew, Weng C. and Ryu, Christopher J.},
  journal = {Phys. Rev. A},
  volume = {107},
  issue = {6},
  pages = {063702},
  numpages = {16},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.107.063702},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.107.063702}
}
@article{Na2020quantumInfoPreserving,
  title = {Quantum information preserving computational electromagnetics},
  author = {Na, Dong-Yeop and Zhu, Jie and Chew, Weng C. and Teixeira, Fernando L.},
  journal = {Phys. Rev. A},
  volume = {102},
  issue = {1},
  pages = {013711},
  numpages = {10},
  year = {2020},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.102.013711},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.102.013711}
}
@article{Miano2025SpectralDensities,
  title = {Spectral densities of a dispersive dielectric sphere in the modified Langevin noise formalism},
  author = {Miano, Giovanni and Cangemi, Loris Maria and Forestiere, Carlo},
  journal = {Phys. Rev. A},
  volume = {112},
  issue = {3},
  pages = {033712},
  numpages = {13},
  year = {2025},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/g71y-hglg},
  url = {https://link.aps.org/doi/10.1103/g71y-hglg}
}

@article{Drezet2017QuantizingPolaritons,
  title = {Quantizing polaritons in inhomogeneous dissipative systems},
  author = {Drezet, Aur\'elien},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {2},
  pages = {023831},
  numpages = {27},
  year = {2017},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.023831},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.95.023831}
}
@article{DiStefano2001ModeExpansion,
author = {Omar Di Stefano and Salvatore Savasta and Raffaello Girlanda},
title = {Mode expansion and photon operators in dispersive and absorbing dielectrics},
journal = {Journal of Modern Optics},
volume = {48},
number = {1},
pages = {67--84},
year = {2001},
publisher = {Taylor \& Francis},
doi = {10.1080/09500340108235155},
}

@article{Gruner1996QEDEvanescent,
  title = {Green-function approach to the radiation-field quantization for homogeneous and inhomogeneous Kramers-Kronig dielectrics},
  author = {Gruner, T. and Welsch, D.-G.},
  journal = {Phys. Rev. A},
  volume = {53},
  issue = {3},
  pages = {1818--1829},
  numpages = {0},
  year = {1996},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.53.1818},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.53.1818}
}
@article{Dung2000QEDLocalized,
  title = {Spontaneous decay in the presence of dispersing and absorbing bodies: General theory and application to a spherical cavity},
  author = {Dung, Ho Trung and Kn\"oll, Ludwig and Welsch, Dirk-Gunnar},
  journal = {Phys. Rev. A},
  volume = {62},
  issue = {5},
  pages = {053804},
  numpages = {13},
  year = {2000},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.62.053804},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.053804}
}
@ARTICLE{Scheel2008MacroscopicQED,
  author  = {S. Scheel and S. Y. Buhmann},
  title   = {Macroscopic Quantum Electrodynamics – Concepts and Applications},
  journal = {Acta Physica Slovaca},
  year    = {2008},
  volume  = {58},
  number  = {5},
  pages   = {675--809}
}

@ARTICLE{Roth2021JMMCT,
  author={Roth, Thomas E. and Chew, Weng C.},
  journal={IEEE Journal on Multiscale and Multiphysics Computational Techniques}, 
  title={Macroscopic Circuit Quantum Electrodynamics: A New Look Toward Developing Full-Wave Numerical Models}, 
  year={2021},
  volume={6},
  number={},
  pages={109-124},
  keywords={Josephson junctions;Qubit;Integrated circuit modeling;Numerical models;Superconducting microwave devices;Junctions;Mathematical model;Circuit quantum electrodynamics;computational electromagnetics;quantum mechanics},
  doi={10.1109/JMMCT.2021.3112808}}
@article{Khan2024PRApplied,
  title = {Field-based formalism for calculating multiqubit exchange-coupling rates for transmon qubits},
  author = {Khan, Ghazi and Roth, Thomas E.},
  journal = {Phys. Rev. Appl.},
  volume = {22},
  issue = {6},
  pages = {064084},
  numpages = {15},
  year = {2024},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.22.064084},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.22.064084}
}
@ARTICLE{Moon2024TAP,
  author={Moon, Soomin and Na, Dong-Yeop and Roth, Thomas E.},
  journal={IEEE Transactions on Antennas and Propagation}, 
  title={Analytical Quantum Full-Wave Solutions for a 3-D Circuit Quantum Electrodynamics System}, 
  year={2024},
  volume={72},
  number={8},
  pages={6702-6716},
  keywords={Qubit;Quantization (signal);Quantum computing;Three-dimensional displays;Antennas and propagation;Superconducting microwave devices;Quantum state;Antenna theory;cavity perturbation theory;circuit quantum electrodynamics (cQED);microwave resonators;quantum theory;transmon qubit},
  doi={10.1109/TAP.2024.3427362}}
@article{Forestiere2023PRA,
  title = {Integral formulation of the macroscopic quantum electrodynamics in dispersive dielectric objects},
  author = {Forestiere, Carlo and Miano, Giovanni},
  journal = {Phys. Rev. A},
  volume = {107},
  issue = {6},
  pages = {063705},
  numpages = {12},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.107.063705},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.107.063705}
}
@article{Ryu2023MPS,
  title = {Matrix product states and numerical mode decomposition for the analysis of gauge-invariant cavity quantum electrodynamics},
  author = {Ryu, Christopher J. and Na, Dong-Yeop and Chew, Weng C.},
  journal = {Phys. Rev. A},
  volume = {107},
  issue = {6},
  pages = {063707},
  numpages = {16},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.107.063707},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.107.063707}
}
@article{Ryu2023Dicke,
  title = {Efficient tensor-network simulation for the few-atom multimode Dicke model via coupling-matrix transformation},
  author = {Ryu, Christopher J. and Na, Dong-Yeop and Chew, Weng C. and Kudeki, Erhan},
  journal = {Phys. Rev. A},
  volume = {108},
  issue = {4},
  pages = {043707},
  numpages = {7},
  year = {2023},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.108.043707},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.108.043707}
}
@article{Dzsotjan2016Modeselective,
  title = {Mode-selective quantization and multimodal effective models for spherically layered systems},
  author = {Dzsotjan, D. and Rousseaux, B. and Jauslin, H. R. and des Francs, G. Colas and Couteau, C. and Gu\'erin, S.},
  journal = {Phys. Rev. A},
  volume = {94},
  issue = {2},
  pages = {023818},
  numpages = {15},
  year = {2016},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.94.023818},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.94.023818}
}
@article{Feist2020Emittercenteredmode,
url = {https://doi.org/10.1515/nanoph-2020-0451},
title = {Macroscopic QED for quantum nanophotonics: emitter-centered modes as a minimal basis for multiemitter problems},
title = {},
author = {Johannes Feist and Antonio I. Fernández-Domínguez and Francisco J. García-Vidal},
pages = {477--489},
volume = {10},
number = {1},
journal = {Nanophotonics},
doi = {doi:10.1515/nanoph-2020-0451},
year = {2021},
lastchecked = {2025-11-28}
}

@ARTICLE{Moon2025CQEM,
  author={Moon, Soomin and Khan, Ghazi and Elkin, Samuel T. and Ryu, Christopher J. and Na, Dong-Yeop and Roth, Thomas E.},
  journal={IEEE Antennas and Propagation Magazine}, 
  title={Computational Quantum Electromagnetics: Basic Concepts and Emerging Trends}, 
  year={2025},
  volume={},
  number={},
  pages={2-13},
  keywords={Numerical models;Mathematical models;Information technology;Computational modeling;Quantization (signal);Dispersion;Photonics;Computers;Quantum system;Antennas},
  doi={10.1109/MAP.2025.3610069}}

@article{Forestiere2022PRA,
  title = {Operative approach to quantum electrodynamics in dispersive dielectric objects based on a polarization-mode expansion},
  author = {Forestiere, Carlo and Miano, Giovanni},
  journal = {Phys. Rev. A},
  volume = {106},
  issue = {3},
  pages = {033701},
  numpages = {28},
  year = {2022},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.106.033701},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.106.033701}
}
@misc{huang2025VIE,
      title={Modeling of Far-Field Quantum Coherence by Dielectric Bodies Based on the Volume Integral Equation Method}, 
      author={Chengnian Huang and Hangyu Ge and Yijia Cheng and Zi He and Feng Liu and Wei E. I. Sha},
      year={2025},
      eprint={2508.16471},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2508.16471}, 
}
@ARTICLE{2022RothJMMCT,
  author={Roth, Thomas E. and Chew, Weng C.},
  journal={IEEE Journal on Multiscale and Multiphysics Computational Techniques}, 
  title={Full-Wave Methodology to Compute the Spontaneous Emission Rate of a Transmon Qubit}, 
  year={2022},
  volume={7},
  number={},
  pages={92-101},
  keywords={Qubit;Electromagnetics;Integrated circuit modeling;Spontaneous emission;Josephson junctions;Superconducting transmission lines;Computers;Circuit quantum electrodynamics;computational electromagnetics;spontaneous emission rate;transmon qubit},
  doi={10.1109/JMMCT.2022.3169460}}
@article{Lalanne2018LightInteraction,
author = {Lalanne, Philippe and Yan, Wei and Vynck, Kevin and Sauvan, Christophe and Hugonin, Jean-Paul},
title = {Light Interaction with Photonic and Plasmonic Resonances},
journal = {Laser \& Photonics Reviews},
volume = {12},
number = {5},
pages = {1700113},
keywords = {cavity perturbation theory, electromagnetic resonance, Fano resonance, LDOS, microcavities, mode volumes, nanoantennas},
doi = {https://doi.org/10.1002/lpor.201700113},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.201700113},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/lpor.201700113},
year = {2018}
}

@article{Kristensen2020Modes,
author = {Kristensen, Philip Trøst and Hughes, Stephen},
title = {Modes and Mode Volumes of Leaky Optical Cavities and Plasmonic Nanoresonators},
journal = {ACS Photonics},
volume = {1},
number = {1},
pages = {2-10},
year = {2014},
doi = {10.1021/ph400114e},
}
@BOOK{Vassallo1991OpticalWaveguide,
  author        = {C. Vassallo},
  title         = {Optical Waveguide Concepts},
  publisher     = {Elsevier},
  year          = {1991}
}
@article{Ching1998QNMs,
  title = {Quasinormal-mode expansion for waves in open systems},
  author = {Ching, E. S. C. and Leung, P. T. and Maassen van den Brink, A. and Suen, W. M. and Tong, S. S. and Young, K.},
  journal = {Rev. Mod. Phys.},
  volume = {70},
  issue = {4},
  pages = {1545--1554},
  numpages = {0},
  year = {1998},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.70.1545},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.70.1545}
}

@ARTICLE{Wu2024DesigningResonators,
  
AUTHOR={Wu, Tong  and Lalanne, Philippe },
         
TITLE={Designing electromagnetic resonators with quasinormal modes},
        
JOURNAL={Frontiers in Physics},
        
VOLUME={Volume 12 - 2024},

YEAR={2024},

URL={https://www.frontiersin.org/journals/physics/articles/10.3389/fphy.2024.1461106},

DOI={10.3389/fphy.2024.1461106},
}

@ARTICLE{wu2024designing,
  
AUTHOR={Wu, Tong  and Lalanne, Philippe },
         
TITLE={Designing electromagnetic resonators with quasinormal modes},
        
JOURNAL={Frontiers in Physics},
        
VOLUME={Volume 12 - 2024},

YEAR={2024},

URL={https://www.frontiersin.org/journals/physics/articles/10.3389/fphy.2024.1461106},

DOI={10.3389/fphy.2024.1461106},
}

@article{chen2017generalizing,
  title = {Generalizing Normal Mode Expansion of Electromagnetic Green's Tensor to Open Systems},
  author = {Chen, Parry Y. and Bergman, David J. and Sivan, Yonatan},
  journal = {Phys. Rev. Appl.},
  volume = {11},
  issue = {4},
  pages = {044018},
  numpages = {19},
  year = {2019},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.11.044018},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.11.044018}
}
@article{sztranyovszky2025extending,
  title = {Extending completeness of the eigenmodes of an open system beyond its boundary, for Green's function and scattering-matrix calculations},
  author = {Sztranyovszky, Z. and Langbein, W. and Muljarov, E. A.},
  journal = {Phys. Rev. Res.},
  volume = {7},
  issue = {1},
  pages = {L012035},
  numpages = {6},
  year = {2025},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.7.L012035},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.7.L012035}
}
@article{Deinega2014TFSF,
  title = {Self-interaction-free approaches for self-consistent solution of the Maxwell-Liouville equations},
  author = {Deinega, Alexei and Seideman, Tamar},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {2},
  pages = {022501},
  numpages = {9},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.022501},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.89.022501}
}

@Article{Chew2019GF,
 authors={Weng Cho Chew, Wei E. I. Sha, Qi Dai},
 title={GREEN'S DYADIC, SPECTRAL FUNCTION, LOCAL DENSITY OF STATES, AND FLUCTUATION DISSIPATION THEOREM},
 volume={166},
 journal={},
 year={2019},
 pages={147-165},
 doi={10.2528/PIER19111801}
 }

@article{Noda2007photonic,
author = {Noda, Susumu and Fujita, Masayuki and Asano, Takashi},
year = {2007},
month = {08},
pages = {},
title = {Spontaneous-emission control by photonic crystals and nanocavities},
volume = {1},
journal = {Nature Photonics},
doi = {10.1038/nphoton.2007.141}
}

@misc{zhou2024simulating,
      title={Simulating quantum emitters in arbitrary photonic environments using FDTD: beyond the semi-classical regime}, 
      author={Qingyi Zhou and S. Ali Hassani Gangaraj and Ming Zhou and Zongfu Yu},
      year={2025},
      eprint={2410.16118},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2410.16118}, 
}
@article{Akimov2007,
  author = {Akimov, A. V. and Mukherjee, A. and Yu, C. L. and Chang, D. E. and Zibrov, A. S. and Hemmer, P. R. and Park, H. and Lukin, M. D.},
  year = {2007},
  title = {Generation of single optical plasmons in metallic nanowires coupled to quantum dots},
  journal = {Nature},
  volume = {450},
  number = {7168},
  pages = {402--406},
  doi = {10.1038/nature06230},
  url = {https://doi.org/10.1038/nature06230}
}
@ARTICLE{Roth2025LorenzGauge,
  author={Elkin, Samuel T. and Sandoval, Felipe and Roth, Thomas E.},
  journal={IEEE Transactions on Antennas and Propagation}, 
  title={Improvements in Wideband and Robust Lorenz Gauge Potential-Based Finite Element Methods}, 
  year={2025},
  volume={},
  number={},
  pages={1-1},
  keywords={Finite element analysis;Geometry;Electric breakdown;Time-domain analysis;Multiphysics;Mathematical models;Integrated circuit modeling;Computers;Antennas and propagation;Vectors;Finite element method;multiscale modeling;low-frequency breakdown;electromagnetic potentials},
  doi={10.1109/TAP.2025.3611588}}

@ARTICLE{Roth2024FullwaveQED,
  author={Moon, Soomin and Na, Dong-Yeop and Roth, Thomas E.},
  journal={IEEE Transactions on Antennas and Propagation}, 
  title={Analytical Quantum Full-Wave Solutions for a 3-D Circuit Quantum Electrodynamics System}, 
  year={2024},
  volume={72},
  number={8},
  pages={6702-6716},
  keywords={Qubit;Quantization (signal);Quantum computing;Three-dimensional displays;Antennas and propagation;Superconducting microwave devices;Quantum state;Antenna theory;cavity perturbation theory;circuit quantum electrodynamics (cQED);microwave resonators;quantum theory;transmon qubit},
  doi={10.1109/TAP.2024.3427362}}
@book{Jin2014FEM,
  author    = {Jian-Ming Jin},
  title     = {The Finite Element Method in Electromagnetics},
  edition   = {3rd},
  publisher = {Wiley-IEEE Press},
  year      = {2014},
  address   = {Hoboken, NJ},
  isbn      = {978-1-118-57125-9}
}

@article{Teixeira2023FDTD,
  author = {Teixeira, F. L. and Sarris, C. and Zhang, Y. and Na, D.-Y. and Berenger, J.-P. and Su, Y. and Okoniewski, M. and Chew, W. C. and Backman, V. and Simpson, J. J.},
  year = {2023},
  title = {Finite-difference time-domain methods},
  journal = {Nature Reviews Methods Primers},
  volume = {3},
  number = {1},
  pages = {75},
  issn = {2662-8449},
  doi = {10.1038/s43586-023-00257-4},
  url = {https://doi.org/10.1038/s43586-023-00257-4}
}
@article{Sohn2025microring,
  title = {Simulating quantum light in lossy microring resonators driven by strong pulses},
  author = {Kim, Youngbin and Jeon, Seongjin and Sohn, Young-Ik},
  journal = {Phys. Rev. Appl.},
  volume = {23},
  issue = {5},
  pages = {054045},
  numpages = {24},
  year = {2025},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.23.054045},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.23.054045}
}
@article{Sohn2024Integrated,
  title = {Simulation of integrated nonlinear quantum optics: From nonlinear interferometer to temporal walk-off compensator},
  author = {Kim, Seonghun and Kim, Youngbin and Yoon, Young-Do and Jeon, Seongjin and Kim, Woo-Joo and Sohn, Young-Ik},
  journal = {Phys. Rev. Appl.},
  volume = {22},
  issue = {6},
  pages = {064092},
  numpages = {37},
  year = {2024},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.22.064092},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.22.064092}
}
@article{Franke_PRL_QNMQuantization_2019,
  title = {Quantization of Quasinormal Modes for Open Cavities and Plasmonic Cavity Quantum Electrodynamics},
  author = {Franke, Sebastian and Hughes, Stephen and Dezfouli, Mohsen Kamandar and Kristensen, Philip Tr\o{}st and Busch, Kurt and Knorr, Andreas and Richter, Marten},
  journal = {Phys. Rev. Lett.},
  volume = {122},
  issue = {21},
  pages = {213901},
  numpages = {6},
  year = {2019},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.122.213901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.122.213901}
}
@article{Bouten2004,
  title = {Stochastic Schr\"{o}dinger equations},
  volume = {37},
  ISSN = {1361-6447},
  url = {http://dx.doi.org/10.1088/0305-4470/37/9/010},
  DOI = {10.1088/0305-4470/37/9/010},
  number = {9},
  journal = {Journal of Physics A: Mathematical and General},
  publisher = {IOP Publishing},
  author = {Bouten,  Luc and Guta,  Madalin and Maassen,  Hans},
  year = {2004},
  month = feb,
  pages = {3189–3209}
}


@article{PRA_twophoton_2025,
  title = {Two-photon superradiance and subradiance},
  author = {Xie, Wenxuan and Mirza, Imran M. and Schotland, John C.},
  journal = {Phys. Rev. A},
  volume = {112},
  issue = {4},
  pages = {043712},
  numpages = {20},
  year = {2025},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/dbny-pjqc},
  url = {https://link.aps.org/doi/10.1103/dbny-pjqc}
}

@article{Gu_PRA_twophoton_2024,
  title = {Two-photon dynamics in non-Markovian waveguide QED with a giant atom},
  author = {Gu, Wenju and Li, Tao and Tian, Ye and Yi, Zhen and Li, Gao-xiang},
  journal = {Phys. Rev. A},
  volume = {110},
  issue = {3},
  pages = {033707},
  numpages = {13},
  year = {2024},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.110.033707},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.110.033707}
}

@article{ECM_nanophotonics_2021,
url = {https://doi.org/10.1515/nanoph-2020-0451},
title = {Macroscopic QED for quantum nanophotonics: emitter-centered modes as a minimal basis for multiemitter problems},
title = {},
author = {Johannes Feist and Antonio I. Fernández-Domínguez and Francisco J. García-Vidal},
pages = {477--489},
volume = {10},
number = {1},
journal = {Nanophotonics},
doi = {doi:10.1515/nanoph-2020-0451},
year = {2021},
lastchecked = {2026-03-22}
}
@article{lambda_advanced_2025,
author = {Zheng, Jun-Cong and Zheng, Xiao-Wei and Hei, Xin-Lei and Qiao, Yi-Fan and Yao, Xiao-Yu and Pan, Xue-Feng and Ren, Yu-Meng and Huo, Xiao-Wen and Li, Peng-Bo},
title = {Non-Markovian Dynamics with $\Lambda$-Type Atomic Systems in a Single-End Photonic Waveguide},
journal = {Advanced Quantum Technologies},
volume = {8},
number = {10},
pages = {2500133},
keywords = {interference, non-markovian dynamics, single-end photonic waveguide, spontaneous emission},
doi = {https://doi.org/10.1002/qute.202500133},
url = {https://advanced.onlinelibrary.wiley.com/doi/abs/10.1002/qute.202500133},
year = {2025}
}

@article{ciatonni_MLN_2024,
  title = {Quantum electrodynamics of lossy magnetodielectric samples in vacuum: Modified Langevin noise formalism},
  author = {Ciattoni, A.},
  journal = {Phys. Rev. A},
  volume = {110},
  issue = {1},
  pages = {013707},
  numpages = {20},
  year = {2024},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.110.013707},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.110.013707}
}
@misc{ciattoni_MLN_2026,
      title={Direct derivation of the modified Langevin noise formalism from the canonical quantization of macroscopic electromagnetism}, 
      author={Alessandro Ciattoni},
      year={2026},
      eprint={2603.04336},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2603.04336}, 
}
@misc{seo_nano_2025,
      title={Quantum-Plasmonic Dynamics Modeled via a Modified Langevin Noise Formalism: Numerical Studies of Single-Photon Emission and Two-Photon Interference}, 
      author={Jisang Seo and Hyunwoo Choi and Thomas E Roth and Jie Zhu and Weng C Chew and Dong-Yeop Na},
      year={2025},
      eprint={2205.03388},
      archivePrefix={arXiv},
      primaryClass={physics.optics},
      url={https://arxiv.org/abs/2205.03388}, 
}
@book{taflove_fdtd,
author = {Taflove, Allen and Hagness, S.},
year = {2000},
month = {06},
pages = {},
title = {Computational electrodynamics: the finite-difference time-domain method. 2nd ed},
volume = {67–106},
isbn = {1-58053-076-1}
}

@article{PRA_ESBESD_2009,
  title = {Sudden death and sudden birth of entanglement in common structured reservoirs},
  author = {Mazzola, L. and Maniscalco, S. and Piilo, J. and Suominen, K.-A. and Garraway, B. M.},
  journal = {Phys. Rev. A},
  volume = {79},
  issue = {4},
  pages = {042302},
  numpages = {4},
  year = {2009},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.79.042302},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.79.042302}
}

@article{PRA_twophoton_2014,
  title = {Strongly correlated two-photon transport in a one-dimensional waveguide coupled to a weakly nonlinear cavity},
  author = {Xu, Xun-Wei and Li, Yong},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {3},
  pages = {033832},
  numpages = {8},
  year = {2014},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.033832},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.033832}
}

@article{PRA_multiphoton_2008,
  title = {Multiphoton scattering in a one-dimensional waveguide with resonant atoms},
  author = {Yudson, V. I. and Reineker, P.},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {052713},
  numpages = {10},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.052713},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.052713}
}
@article{Reiserer_gate_nature_2014,
  title = {A quantum gate between a flying optical photon and a single trapped atom},
  volume = {508},
  ISSN = {1476-4687},
  url = {http://dx.doi.org/10.1038/nature13177},
  DOI = {10.1038/nature13177},
  number = {7495},
  journal = {Nature},
  publisher = {Springer Science and Business Media LLC},
  author = {Reiserer,  Andreas and Kalb,  Norbert and Rempe,  Gerhard and Ritter,  Stephan},
  year = {2014},
  month = apr,
  pages = {237–240}
}
@misc{elkin_CQEMreview_2025,
      title={Opportunities and Challenges of Computational Electromagnetics Methods for Superconducting Circuit Quantum Device Modeling: A Practical Review}, 
      author={Samuel T. Elkin and Ghazi Khan and Ebrahim Forati and Brandon W. Langley and Dogan Timucin and Reza Molavi and Sara Sussman and Thomas E. Roth},
      year={2025},
      eprint={2511.20774},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2511.20774}, 
}
@article{Chew2024,
  title = {Some Selected Unsolved Problems in Classical and Quantum Electromagnetics},
  volume = {180},
  ISSN = {1559-8985},
  url = {http://dx.doi.org/10.2528/PIER24072910},
  DOI = {10.2528/pier24072910},
  journal = {Progress In Electromagnetics Research},
  publisher = {The Electromagnetics Academy},
  author = {Chew,  Weng Cho and Zhang,  Boyuan and Zhu,  Jie},
  year = {2024},
  pages = {79–87}
}

@article{Huttner1992Quantization,
  title = {Three-dimensional quantization of the electromagnetic field in dispersive and absorbing inhomogeneous dielectrics},
  author = {Dung, Ho Trung and Kn\"oll, Ludwig and Welsch, Dirk-Gunnar},
  journal = {Phys. Rev. A},
  volume = {57},
  issue = {5},
  pages = {3931--3942},
  numpages = {0},
  year = {1998},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.57.3931},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.57.3931}
}
@article{Vidal_PRB_fewmode_2025,
  title = {Photon-mediated interactions and dynamics of coherently driven quantum emitters in complex photonic environments},
  author = {Miguel-Torcal, A. and Gonz\'alez-Tudela, A. and Garc\'{\i}a-Vidal, F. J. and Fern\'andez-Dom\'{\i}nguez, A. I.},
  journal = {Phys. Rev. B},
  volume = {112},
  issue = {23},
  pages = {235419},
  numpages = {9},
  year = {2025},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/syk9-6dny},
  url = {https://link.aps.org/doi/10.1103/syk9-6dny}
}
@article{Dicke_1954,
  title = {Coherence in Spontaneous Radiation Processes},
  author = {Dicke, R. H.},
  journal = {Phys. Rev.},
  volume = {93},
  issue = {1},
  pages = {99--110},
  numpages = {0},
  year = {1954},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.93.99},
  url = {https://link.aps.org/doi/10.1103/PhysRev.93.99}
}
@article{PRA_dicke_2000,
  title = {Three qubits can be entangled in two inequivalent ways},
  author = {D\"ur, W. and Vidal, G. and Cirac, J. I.},
  journal = {Phys. Rev. A},
  volume = {62},
  issue = {6},
  pages = {062314},
  numpages = {12},
  year = {2000},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.62.062314},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.062314}
}

@article{Forestire_PRA_2025,
  title = {Spectral densities of a dispersive dielectric sphere in the modified Langevin noise formalism},
  author = {Miano, Giovanni and Cangemi, Loris Maria and Forestiere, Carlo},
  journal = {Phys. Rev. A},
  volume = {112},
  issue = {3},
  pages = {033712},
  numpages = {13},
  year = {2025},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/g71y-hglg},
  url = {https://link.aps.org/doi/10.1103/g71y-hglg}
}
@article{Pepe_PRR_2025,
  title = {Non-Markovian dynamics of generation of bound states in the continuum via single-photon scattering},
  author = {Magnifico, Giuseppe and Maffei, Maria and Pomarico, Domenico and Das, Debmalya and Facchi, Paolo and Pascazio, Saverio and Pepe, Francesco V.},
  journal = {Phys. Rev. Res.},
  volume = {7},
  issue = {3},
  pages = {033249},
  numpages = {9},
  year = {2025},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/gtf6-zb57},
  url = {https://link.aps.org/doi/10.1103/gtf6-zb57}
}


@article{Forestire_nanophotonics_2025,
url = {https://doi.org/10.1515/nanoph-2024-0703},
title = {Quantum emitter interacting with a dispersive dielectric object: a model based on the modified Langevin noise formalism},
title = {},
author = {Giovanni Miano and Loris Maria Cangemi and Carlo Forestiere},
pages = {4019--4027},
volume = {14},
number = {23},
journal = {Nanophotonics},
doi = {doi:10.1515/nanoph-2024-0703},
year = {2025},
lastchecked = {2026-03-24}
}
@article{miano_ECM_PRA_2026,
  title = {Modified Langevin noise formalism for multiple quantum emitters in dispersive electromagnetic environments out of equilibrium},
  author = {Miano, Giovanni and Cangemi, Loris Maria and Forestiere, Carlo},
  journal = {Phys. Rev. A},
  volume = {113},
  issue = {2},
  pages = {023720},
  numpages = {20},
  year = {2026},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/ps9g-1b4d},
  url = {https://link.aps.org/doi/10.1103/ps9g-1b4d}
}

@article{PRA_wstate_2025,
  title = {High-fidelity generation of Bell and $W$ states in a giant-atom system via bound states in the continuum},
  author = {Weng, Mingzhu and Yu, Hongwei and Wang, Zhihai},
  journal = {Phys. Rev. A},
  volume = {111},
  issue = {5},
  pages = {053711},
  numpages = {7},
  year = {2025},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.111.053711},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.111.053711}
}
@article{PRA_MPS_2025,
  title = {Efficient tensor-network simulation of multiemitter non-Markovian systems},
  author = {Papaefstathiou, Irene and Malz, Daniel and Cirac, J. Ignacio and Ba\~nuls, Mari Carmen},
  journal = {Phys. Rev. A},
  volume = {112},
  issue = {1},
  pages = {013721},
  numpages = {13},
  year = {2025},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/hmbj-lg7p},
  url = {https://link.aps.org/doi/10.1103/hmbj-lg7p}
}
@misc{Giuseppe_MPS_2025,
      title={Superradiant decay in non-Markovian Waveguide Quantum Electrodynamics}, 
      author={Rosa Lucia Capurso and Giuseppe Calajó and Simone Montangero and Saverio Pascazio and Francesco V. Pepe and Maria Maffei and Giuseppe Magnifico and Paolo Facchi},
      year={2025},
      eprint={2511.22332},
      archivePrefix={arXiv},
      primaryClass={quant-ph},
      url={https://arxiv.org/abs/2511.22332}, 
}

@article{PRL_MPS_2016,
  title = {Photonic Circuits with Time Delays and Quantum Feedback},
  author = {Pichler, Hannes and Zoller, Peter},
  journal = {Phys. Rev. Lett.},
  volume = {116},
  issue = {9},
  pages = {093601},
  numpages = {6},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.116.093601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.093601}
}
@article{PRX_MPS_2024,
  title = {Continuous Coherent Quantum Feedback with Time Delays: Tensor Network Solution},
  author = {Vodenkova, Kseniia and Pichler, Hannes},
  journal = {Phys. Rev. X},
  volume = {14},
  issue = {3},
  pages = {031043},
  numpages = {32},
  year = {2024},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.14.031043},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.14.031043}
}


==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2016/06/03 v1.7 Michael Downes]
% Copyright 2000 Michael John Downes
%
% Following Michael's death, his family have requested that his TeX
% related files are made publicly available under the LPPL license.
%
% This file is available under the LaTeX Project Public License version 1
% or (at your option) any later version.
% https://latex-project.org/lppl/
% (LPPL maintenance status: unmaintained)
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa

